WegFormer: Transformers for Weakly Supervised Semantic Segmentation

Although convolutional neural networks (CNNs) have achieved remarkable progress in weakly supervised semantic segmentation (WSSS), the effective receptive field of CNN is insufficient to capture global context information, leading to sub-optimal results. Inspired by the great success of Transformers in fundamental vision areas, this work for the first time introduces Transformer to build a simple and effective WSSS framework, termed WegFormer. Unlike existing CNN-based methods, WegFormer uses Vision Transformer (ViT) as a classifier to produce high-quality pseudo segmentation masks. To this end, we introduce three tailored components in our Transformer-based framework, which are (1) a Deep Taylor Decomposition (DTD) to generate attention maps, (2) a soft erasing module to smooth the attention maps, and (3) an efficient potential object mining (EPOM) to filter noisy activation in the background. Without any bells and whistles, WegFormer achieves state-of-the-art 70.5% mIoU on the PASCAL VOC dataset, significantly outperforming the previous best method. We hope WegFormer provides a new perspective to tap the potential of Transformer in weakly supervised semantic segmentation. Code will be released.

==> WegFormer_ Transformers for weakly supervised semantic segmentation/table/attAblation.tex <==
\begin{tabular}{p{130pt}<{\RaggedRight}p{40pt}<{\centering}}
\toprule
 \rule{0pt}{8pt}\textbf{Blocks} & \textbf{mIoU}\\
\midrule
 \rule{0pt}{8pt}\text{0, 1, 2, 3, 4, 5, 6, 7, 8, 9, 10, 11} & \text{58.2}\\
\midrule
 \rule{0pt}{8pt}\text{3,4,5,6,7,8,9,10,11} & \text{58.4}\\
\midrule
 \rule{0pt}{8pt}\text{5,6,7,8,9,10,11} & \text{58.2}\\
\midrule
 \rule{0pt}{8pt}\text{7,8,9,10,11} & \text{58.8}\\
\midrule
 \rule{0pt}{8pt}\text{9,10,11} & \text{59.0}\\
\midrule
 \rule{0pt}{8pt}\text{11} & \text{59.5}\\
\bottomrule
\end{tabular}

==> WegFormer_ Transformers for weakly supervised semantic segmentation/table/seg.tex <==

\begin{tabular}{p{60pt}<{\raggedright}p{55pt}<{\centering}p{31pt}<{\centering}}

\toprule
 \rule{0pt}{9pt}   \textbf{Network}   & \textbf{val} & \textbf{test}\\
\midrule
 \rule{0pt}{9pt}   \text{DeepLab-V2}  & \text{69.2}  & \text{69.7}\\
\midrule
 \rule{0pt}{9pt}   \text{DeepLab-V3} & \text{69.3}    & \text{69.9}\\
\midrule
 \rule{0pt}{9pt}   \text{DeepLab-V3+} & \text{70.5}  & \text{70.3}\\
\bottomrule
\end{tabular}

==> WegFormer_ Transformers for weakly supervised semantic segmentation/table/sota.tex <==
\begin{tabular}{p{45pt}<{\RaggedRight}p{20pt}<{\centering}p{20pt}<{\centering}p{45pt}<{\RaggedRight}p{20pt}<{\centering}p{20pt}<{\centering}}
% \begin{tabular}{c|c|c|c|c|c}
\toprule
\multicolumn{3}{c|}{ \rule{0pt}{9pt}\textbf{VGG}}                & \multicolumn{3}{c}{\textbf{ResNet}}              \\ \midrule
 \rule{0pt}{9pt}\textbf{Methods} & \textbf{Val}  & \textbf{Test} & \multicolumn{1}{|l}{\textbf{Methods}} & \textbf{Val}  & \textbf{Test} \\ \midrule
 \rule{0pt}{9pt}SEC              & 50.7          & 51.7          &\multicolumn{1}{|l}{DCSP}             & 60.8          & 61.9          \\
 \rule{0pt}{9pt}STC              & 49.8          & 51.2          & \multicolumn{1}{|l}{DSRG}             & 61.4          & 63.2          \\
 \rule{0pt}{9pt}Roy et al.       & 52.8          & 53.7          & \multicolumn{1}{|l}{MCOF}        & 60.3          & 61.2          \\
 \rule{0pt}{9pt}Oh et al.        & 55.7          & 56.7          & \multicolumn{1}{|l}{AffinityNet}      & 61.7          & 63.7          \\
 \rule{0pt}{9pt}AE-PSL           & 55.0          & 55.7          & \multicolumn{1}{|l}{SeeNet}           & 63.1          & 62.8          \\
 \rule{0pt}{9pt}WebS-i2          & 53.4          & 55.3          & \multicolumn{1}{|l}{IRN}              & 63.5          & 64.8          \\
 \rule{0pt}{9pt}Hong et al.      & 58.1          & 58.7          & \multicolumn{1}{|l}{FickleNet}        & 64.9          & 65.3          \\
 \rule{0pt}{9pt}DCSP             & 58.6          & 59.2          & \multicolumn{1}{|l}{OAA}              & 65.2          & 66.4          \\
 \rule{0pt}{9pt}TPL              & 53.1          & 53.8          & \multicolumn{1}{|l}{SSDD}             & 64.9          & 65.5          \\
 \rule{0pt}{9pt}GAIN             & 55.3          & 56.8          & \multicolumn{1}{|l}{SEAM}             & 64.5          & 65.7          \\
 \rule{0pt}{9pt}DSRG             & 59.0          & 60.4          & \multicolumn{1}{|l}{SCE}              & 66.1          & 65.9          \\
 \rule{0pt}{9pt}MCOF             & 56.2          & 57.6          & \multicolumn{1}{|l}{ICD}              & 67.8          & 68.0          \\
 \rule{0pt}{9pt}AffinityNet      & 58.4          & 60.5          & \multicolumn{1}{|l}{Zhang et al.}     & 66.6          & 66.7          \\
 \rule{0pt}{9pt}RDC              & 60.4          & 60.8          & \multicolumn{1}{|l}{Fan et al.}       & 67.2          & 66.7          \\
 \rule{0pt}{9pt}SeeNet           & 63.1          & 62.8          & \multicolumn{1}{|l}{MCIS}             & 66.2          & 66.9          \\
 \rule{0pt}{9pt}OAA              & 63.1          & 62.8          & \multicolumn{1}{|l}{BES}              & 65.7          & 66.6          \\
 \rule{0pt}{9pt}ICD              & 64.0          & 63.9          & \multicolumn{1}{|l}{CONTA}            & 66.1          & 66.7          \\
 \rule{0pt}{9pt}BES              & 60.1          & 61.1          & \multicolumn{1}{|l}{DRS}              & 66.8          & 67.4          \\
 \rule{0pt}{9pt}Fan et al.       & 64.6          & 64.2          & \multicolumn{1}{|l}{NSROM}            & 68.3          & 68.5          \\
 \rule{0pt}{9pt}Zhang et al.     & 63.7          & 64.5          & \multicolumn{1}{|l}{\textbf{Ours}}    & \textbf{70.5} & \textbf{70.3} \\ \cline{4-6} 
 \rule{0pt}{9pt}MCIS             & 63.5          & 63.6          & \multicolumn{1}{|l}{OAA$\dagger$}             & 67.4          & —             \\
 \rule{0pt}{9pt}DRS              & 63.6          & 64.4          & \multicolumn{1}{|l}{\textbf{DRS$\dagger$}}    & \textbf{71.2} & \textbf{71.4} \\
 \rule{0pt}{9pt}NSROM            & 65.5          & 65.3          & \multicolumn{1}{|l}{NSROM$\dagger$}           & 70.4          & 70.2          \\
 \rule{0pt}{9pt}\textbf{Ours}    & \textbf{66.2} & \textbf{66.5} & \multicolumn{1}{|l}{Ours$\dagger$}            & 70.9          & 70.5          \\ \bottomrule
\label{Tab.quan}
\end{tabular}

==> WegFormer_ Transformers for weakly supervised semantic segmentation/table/sumAblation.tex <==

\begin{tabular}{p{42pt}<{\centering}p{35pt}<{\centering}p{46pt}<{\centering}p{30pt}<{\centering}p{18pt}<{\centering}}
\toprule
 \rule{0pt}{8pt} \textbf{Soft Erase}&\textbf{Sal~(DRS)}&\textbf{Sal~(NSROM)}&\textbf{EPOM$\ast$}&\textbf{mIoU}\\
\midrule
 \rule{0pt}{8pt} \text{-} & \text{-} & \text{-} & \text{-} &  \text{59.5}\\
 \rule{0pt}{8pt} \checkmark & \text{-} & \text{-} & \text{-} &  \text{60.0}\\
 \rule{0pt}{8pt} \checkmark & \checkmark & \text{-} & \text{-} & \text{70.2}\\
 \rule{0pt}{8pt} \checkmark & \checkmark & \text{-} & \checkmark & \text{70.9}\\
 \midrule
 \rule{0pt}{8pt} \checkmark & \text{-} & \checkmark & \text{-} & \text{68.9}\\
 \rule{0pt}{8pt} \checkmark & \text{-} & \checkmark & \checkmark & \text{69.8}\\

\bottomrule
\end{tabular}
